KAG: Boosting LLMs in Professional Domains via Knowledge Augmented Generation

The recently developed retrieval-augmented generation (RAG) technology has enabled the efficient construction of domain-specific applications. However, it also has limitations, including the gap between vector similarity and the relevance of knowledge reasoning, as well as insensitivity to knowledge logic, such as numerical values, temporal relations, expert rules, and others, which hinder the effectiveness of professional knowledge services. In this work, we introduce a professional domain knowledge service framework called Knowledge Augmented Generation (KAG). KAG is designed to address the aforementioned challenges with the motivation of making full use of the advantages of knowledge graph(KG) and vector retrieval, and to improve generation and reasoning performance by bidirectionally enhancing large language models (LLMs) and KGs through five key aspects: (1) LLM-friendly knowledge representation, (2) mutual-indexing between knowledge graphs and original chunks, (3) logical-form-guided hybrid reasoning engine, (4) knowledge alignment with semantic reasoning, and (5) model capability enhancement for KAG. We compared KAG with existing RAG methods in multihop question answering and found that it significantly outperforms state-of-theart methods, achieving a relative improvement of 19.6% on 2wiki and 33.5% on hotpotQA in terms of F1 score. We have successfully applied KAG to two professional knowledge Q&A tasks of Ant Group, including E-Government Q&A and E-Health Q&A, achieving significant improvement in professionalism compared to RAG methods.

==> secs/data-model.tex <==
\section{The OneGraph Model}
\label{sec:data-model}
\begin{table}[]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|l}
    \toprule
     & Interpretation \\
     \midrule
     Object & The things included in the OneGraph data, such as named entities. \\
     Head Object (Head) & The first element of a triple.  \\
     Relation Object (Relation) & The second element of a triple. \\
     Tail Object (Tail) & The third element of a triple. \\
     Name & The name of an entity. \\
     Description &  \\
     Document & \\
     \bottomrule
    \end{tabular}
    }
    \caption{Vocabulary.}
    \label{tab:vocabulary}
\end{table}
\subsection{Structure}
\paragraph{All objects are represented as text.} In the OneGraph model, all things including beings (e.g. people, organization, concepts) and relations are represented as text. For example, $\texttt{Albert Einstein}$ denotes the famous scientist Albert Einstein. $\texttt{has won prize}$ denotes a relation that some one has won a prize. 

\paragraph{Two text can have relations, composing a triple.} For example, the following triple
$$ \texttt{Albert Einstein} \sep \texttt{has won prize} \sep \texttt{Nobel Prize}  $$
denotes the fact that Albert Einstein has won the Nobel Prize. We use $\square$ to separate the text, which is less likely to be used in a normal natural language text. 

\paragraph{Each text in the OneGraph model is labeled as \texttt{Name, Description, Document} from the perspective of text.} \texttt{Name} denotes a few words that named the beings and relations. For example, if we want to say that $\texttt{Albert Einstein}$ is the name of the scientist Albert Einstein,  it could be expressed as
$$ \texttt{Albert Einstein} \sep \texttt{text label} \sep \texttt{Name}$$
We use the $\texttt{text label}$ to denote the text label of the object.
\texttt{Description} is a few words that could describe the object we want to store. \texttt{Red and Long Dress} describe a kind of dress, and we will label it by the following triple
$$ \texttt{Red and Long Dress} \sep \texttt{text label}\sep \texttt{Description}$$ 
\texttt{Document} is a long text composed by one or more sentences. For example, we could label a well-known sentences from fictions as $\texttt{Document}$ that 
$$\texttt{To be, or not to be, that is the question.} \sep \texttt{text label} \sep \texttt{Document}$$
\paragraph{Each text is as also labeled as \texttt{String}, \texttt{time}, \texttt{Number} from the perspective of formate.} For example, to state that Albert Einstein is born in 1879, we write:
\begin{align}
& \texttt{Albert Einstein} \sep \texttt{born in} \sep \texttt{1879} \nonumber\\
&\texttt{1879} \sep \texttt{format label} \sep \texttt{time} \nonumber
\end{align}

To deal with synonymy and ambiguity, for example, both \texttt{ZJU} and \texttt{Zhejiang University} could represent Zhejiang University. We define a specific text type \texttt{Abstract} to represent the unique objects, for example
\begin{align}
    & \texttt{ZJU} \sep \texttt{abstract to} \sep \texttt{Chinese University-ZJU} \nonumber\\
    & \texttt{Chinese University-ZJU} \sep \texttt{text type} \sep \texttt{Abstract} \nonumber
\end{align}
\texttt{Chinese University-ZJU} is an abstract text used to represent the Zhejiang University. Different to other types of text, in all abstract text, there will not be two abstract texts represent the same object. Each object has a unique and only one abstract text. Thus the function of abstract text is similar to the URI in the traditional data model of ontology such as RDF. 

\paragraph{Texts could be grouped into classes represented as text.} For example, \texttt{University} is composed by all universities in the world. We use \texttt{type} to denote the class-instance relation that 
$$ \texttt{Zhejiang University} \sep \texttt{type} \sep \texttt{University} $$
The class could also be in instance of another class. For example
$$ \texttt{University} \sep \texttt{type} \sep \texttt{Educational Institution}$$
With the \texttt{type} relation, classes and entities are organized in a hierarchy. We do not distinguish the type relation between entities and classes and between classes and classes.  
For each class, we label it as \texttt{Complete} or \texttt{Incomplete}. \texttt{Complete} denotes the instances or subclasses of the class is stored in the data. For example
\begin{align}
& \ttt{Francesca Rossi} \sep \ttt{type} \sep \ttt{ISWC2022 Keynot Speaker} \nonumber \\
& \ttt{Ilaria Capua} \sep \ttt{type} \sep \ttt{ISWC2022 Keynot Speaker} \nonumber \\
& \ttt{Markus Krötzsch} \sep \ttt{type} \sep \ttt{ISWC2022 Keynot Speaker} \nonumber \\
& \ttt{ISWC2022 Keynot Speaker} \sep \ttt{class type} \sep \ttt{Complete} \nonumber
\end{align}
These triples means that there are 3 keynote speaker in ISWC2022 and all of them are stored in the data. 

\texttt{Incomplete} means not all instances or subclasses are recorded. Each class is labeled as \texttt{Incomplete} by default. For example if only one keynote speaker is known in the previous example, the data will be 
\begin{align}
& \ttt{Francesca Rossi} \sep \ttt{type} \sep \ttt{ISWC2022 Keynot Speaker} \nonumber \\
& \ttt{ISWC2022 Keynote Speaker} \sep \ttt{class label} \sep \ttt{Incomplete} \nonumber
\end{align}

In the OneGraph model, all texts could be the subject, relation, and object in the triple. This allows to represent the properties of relations and relations between relations. For example, we could define one relation is a sub-relation of the other one like
$$ \texttt{has father} \sep \texttt{sub-relation of} \sep \texttt{has parents}$$

For complex events that could not be expressed in a single fact. We make a triple also as   

We use multiple triples with abstract text to represented it. To express the event that OpenAI introduced ChatGPT, we make a triple also as an object, and link it to the subject, relation, object. 
\begin{align}
& \ttt{OpenAI} \sep \ttt{announced} \sep \ttt{ChatGPT} \nonumber \\
& \ttt{OpenAI announced ChatGPT} \sep \ttt{subject} \sep \ttt{OpenAI} \\
& \ttt{OpenAI announced ChatGPT} \sep \ttt{relation} \sep \ttt{announced} \\
& \ttt{OpenAI announced ChatGPT} \sep \ttt{object} \sep \ttt{ChatGPT} \\
& \ttt{OpenAI announced ChatGPT} \sep \ttt{date} \sep \ttt{2022.11.30} \\
& \ttt{OpenAI announced ChatGPT} \sep \ttt{introducing blog} \sep \ttt{https://openai.com/blog/chatgpt} \nonumber \\ 
& \ttt{OpenAI announced ChatGPT} \sep \ttt{text type} \sep \ttt{description} \\
\end{align}


 

\subsection{Discussion}
Previous data model in the KG projects are designed to be language-independent. While the OneGraph model is language-dependent and language-friendly.

We do not require each entity to be an instance of at least of one class. 

OneGraph Model supports: edge property, which is not supported by RDF and RDF-star. 






\subsection{Semantics}
In this section, we will give a model-theoretic semantics to OneGraph. We first precribe that the set of objects $\mathcal{O}$ for any OneGraph model must contain  \ttt{type, text label, format label, class label, abstract to} as relation objects, \ttt{Name, Description, Document}, \ttt{Abstract, Complete, Incomplete} for head and tail object. 

\subsection{Relation to Other Formalisms}


==> secs/evaluation.tex <==
\section{Evaluation}


==> secs/improve-accuracy.tex <==
\section{Constructing Higher Accuracy LLMKG}

==> secs/improve-coverage.tex <==
\section{Constructing Higher Coverage LLMKG}

==> secs/overview.tex <==
\section{Overview of OneGraph}
In this section, we present our vision of knowledge augmented LLMs, from which we realize the necessary of LLMKG,  and the overview of constructing process of the LLMKG we tried. The overview is shown in Figure \ref{fig:overview}. 

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/overview.pdf}
    \caption{Overview of the process of constructing LLMKG (the OneGraph in this work) and utilizing LLMKG.}
    \label{fig:overview}
\end{figure}

\subsection{Vision of Knowledge Augmented LLMs}
The capability of AI systems with large language model only is limited. There are hallucinations and  out-of-date knowledge issues. There is max length limitation for the input text. Though many hard works are tried to enable longer and longer input text, the max length limitation still exists. Thus we can't input big data, such as large scale knowledge graphs, into the large language model. If the data is not included in the training dataset of the LLMs or has different distribution compared to the training data of the LLMs, extra modules to corporate with LLMs to enable them to fully utilize these data is necessary. Inspired by the phrase ``knowledge representation and reasoning", we think there should be two extra modules: a knowledge memory module (corresponding to knowledge representation) and a knowledge inference module (corresponding to knowledge reasoning). 
\begin{itemize}
    \item \textit{Knowledge Memory Module}: The knowledge memory module is to accurately memorize (or represent) the knowledge that LLMs need to be interact with during output generation. Considering the success of both symbolic knowledge representation and the parametric knowledge representation, we think there should two sub-modules: \textit{the LM-as-KG sub-module} that maintains a language-model-based model, which might not necessarily be very large, to service as a parametric knowledge graph; \textit{the LLMKG sub-module} symbolically represent the extra knowledge needed for LLMs to generate the output. The content in the LLMKG could be injected into the LM-as-KG sub-module, and the contents of the LLMKG and the LM-as-KG sub-module could be mostly the same via alignment methods. Apart from the accuracy of knowledge, the knowledge memory module is expected to also have the following properties: easy to maintain including deleting, updating and adding knowledge; record the provenance of the knowledge.  
    \item \textit{Knowledge Inference Module}: The knowledge inference module takes the responsibility of conducting inference over the knowledge included in the knowledge memory module, such as extracting the related knowledge, inferring the missing knowledge, and abstract the relevant knowledge based on the requirements from the LLMs. This module could be composed by a \textit{LM-as-Reasoner} model which could be  language-model-based and acting as a reasoner that could take full utilization and manipulation over the knowledge stored in the knowledge memory module. The LM-as-Reasoner model will constantly interact with the LM-as-KG model and the LLMKG to get the latest and accurate knowledge. The expected feature of the knowledge inference modules are: could translate the LLMs requirements into knowledge requirements; could meet the knowledge requirements by querying and reasoning over the knowledge memory module; is capable of conduct complex logic reasoning over knowledge.  
\end{itemize}

Combining large language model with the knowledge inference module and the knowledge memory module could make the LLMs:
\begin{itemize}
    \item More trustful: LLMs will utilize the accurate and up-to-date related knowledge to generate the output.  
    \item More controllable: The output of the LLMs depends on the knowledge in the memory module which is easy to maintain. Thus it is possible to manipulate the LLMs' output by updating the knowledge in the memory module. 
    \item More powerful: The symbolic represented LLMKG could store huge amount of knowledge. With these external and easy access knowledge resource, LLMs could complete more tasks than with LLMs only.  
\end{itemize}

For knowledge augmented LLMs, both the knowledge inference module and the knowledge memory module are important. Considering the LLM-as-Reasoner model and the LLM-as-KG model depend on the LLMKG, we realize that LLMKG is the basis of the framework and should be explored as the first step of achieving the knowledge augmented LLMs. Thus we made our first trial to construct an LLMKG. We call it OneGraph, with the expectation of included knowledge that is useful for LLMs as much as possible in one LLMKG. Next we introduce the overview of the OneGraph constructing process. 

\subsection{OneGraph Constructing Process}
Before constructing the LLMKG, we list the following expectations for the construction:
\begin{itemize}
    \item High Accuracy: The knowledge stored in the LLMKG should be as accurate as possible. If the wrong knowledge in the LLMKG be used to enhance the LLMs, it might worsen the performance of LLMs. At least the accuracy of knowledge stored in the LLMKG should be higher than the accuracy of knowledge embodied in the LLMs.  
    \item High Coverage: The coverage of knowledge in LLMKG should be as high as possible. This ensures the LLMKG is helpful for LLMs in applications of diverse domains. Thus it is not a KG constructed to improve the capability of LLMs in a specific domain but to improve the general capability across domains. 
    % \item In a Text-rich Form: The LLMKG should be represented in a LLM-friendly way, which means it should be represented in a way making it easy to be applied to LLMs. Thus LLMKG should be text-rich. For example, with a piece of text attached to all the elements in the LLMKG. 
    \item Low Cost: The cost of mainly includes financial cost and time cost. The low financial cost per triple ensures that construction large LLMKG is affordable. The low time cost for construction ensures that an LLMKG could be quickly been constructed if necessary. 
\end{itemize}

To achieve this, we take full 







==> secs/related-works.tex <==
\section{Related Works}
In this section, we mainly introduce the related works using LLMs for KG construction. 


\input{tables/comparison}


\subsection{LM-as-KB Paradigm}
The first study of in-depth analysis of the relational knowledge present in the pretrained language model is \cite{llmaskb}. Authors show that language models could answer the queries structured as ``fill-in-the-blank" cloze statements, such as ``Dante was birn in [MASK]" to predict what is the mask token. The question ``Language models as knowledge based?" (LM-as-KB) is firstly proposed, which is also the title of the work \cite{llmaskb}. The language models have many advantages over the symbolic and structured knowledge base, which are schema-free requiring no schema engineering and are able to handle open class of relations.  The LAMA (LAnguage Model Analysis) probe benchmark is introduced and widely used to test the factual and commonsense knowledge in the language model. Since then, a stirred discussion as to what extend language model could be an alternative to, or at least be a proxy for explicit knowledge bases is conducted. \cite{llmaskborforkb} further discuss the difference between the LM-as-KB paradigm and the structured KB paradigm from the perspective of construction, schema, maintenance, knows what it knows, etc, as shown in Table \ref{tab:difference}\footnote{We do not include the  perspective of entity disambiguation in Table \ref{tab:difference} which is included in the original table in \cite{llmaskborforkb}, since the large language models in now-days such as GPT 3.5/4 are also commonly good at entity disambiguation. }. In Table \ref{tab:difference}, we also add LLMKG into comparison. As we can see, the LM-as-KB could be constructed in a self/Unsupervised way and is schema-free. And the conventional structured KBs are easy to maintain, has a clear knowledge border that knows what it knows, and has the ability to trace the origin of the knowledge by keeping the reference sources. While the LLMKG, we are interested in this paper, keeps the advantages of the LM-as-KB paradigm and the conventional structured KB. It is a schema-free structured KGs constructed based on language models. 

Though empirical experiments shows the potential of LM-as-KB paradigm, some works question this paradigm and point out the shortcoming of this paradigm. 
\cite{llmaskb-guess} shows that pre-trained masked language models are making educated guessing when filling the mask and the performance of prompt-based paradigm is prompt-biased. The improvements by incorporating illustrative cases and external contexts is mainly due to entity type guidance and golden answer leakage. 
\cite{head-to-tail} explore how knowledgeable are LLMs by constructing a benchmark Head-to-Tail consists of 18k question-answer pairs of head, torso, and tail facts in terms of popularity, and it shows that existing LLMs including GPT4 are still far from being perfect in terms of remembering of factual knowledge, especially for facts of torso-to-tail entities. The accuracy of question answering over open and specific domains of the tail entities is only $27.3\%$ and $10.6\%$ respectively, which is quite low, and is apparently not enough to support regarding LLMs as knowledgeable for tail entities. 
\cite{lmastkg} points that it is still challenging for LMs to memorize conflicting information which also hinders the memorization of other unrelated one-to-one relationships.

Apart from directly regarding the LM trained on vast text corpus as knowledge base, the LM-as-KB paradigm could also be achieved by post training to enable language models memorizing and reasoning among large scale knowledge base. 
Starting from the pre-trained checkpoints of open-source language models including T5 and LLaMA-2, \cite{lmmemorizekb} continue train these language models on a filtered Wikidata containing 46M triples. Experiment results show that LMs are capable of memorizing triples in knowledge base at large scale, and the larger the model is, the quicker it learns. But the infrequent knowledge is more challenging to memorize, irrespective of the language model size. It also shows language model trained on knowledge based are better at retrieving and organizing long-tail knowledge when answering questions related to long-tail knowledge.  Further more, experiments on missing facts prediction shows that the fine-tuned language models are capable of inferring missing entities of triples from existing knowledge to some extent and struggle with inverse reasoning.  

These works proves the language models could serve as the knowledge base to some extend. However, their knowledge probing performance will be affected by the form of prompts. They are struggle to memorize triples about long-tail entities and relations, conflict information such as triples about 1-N, N-N relations, and has limited reasoning capabilities over triples, this shortcomings still exists after post-training the language model with corpus from existing knowledge bases. Thus language models cannot replace symbolic knowledge base as a trustful knowledge resources. Thus more and more works investigate how the enable large language models and knowledge graphs benefit each other.         

\subsection{LLM for KG Construction}
A lot of knowledge graphs have been constructed and are assets for recommender system, search engine and other applications. However, they are far from complete. Thus 
constructing accurate and complete structured knowledge graphs is challenging.
\cite{llm4kbc} explored the potential of GPT models for knowledge base completion. It shows involvement of language model for completion significantly reduce the construction cost and with proper thresholding, GPT-3 successfully extend Wikidata by 27M facts at $90\%$ precision, showing the effectiveness of large language model for knowledge graph completion. However, it also reveals that language model do not produce statements of a high enough accuracy, which achieve a quite low recall, ranging from $0.01$ to $0.70$, when constrain the precision to be high such as above $90\%$ or $95\%$. 
Missing triples could also be inferred based on the graph structures, 
\cite{kopa} propose a method KoPA to incorporate the structural information of knowledge graphs into large language models. KoPA includes a knowledge prefix adapter to which projects structural embeddings into textual space and obtains virtual knowledge tokens positioned as a prefix of the input prompt. KoPA shows better link prediction performance over embedding-based, PLM-based, training-free LLM-based, and fine-tuning LLM-based baselines. 
\cite{DBLP:conf/coling/WangHHLYL24} focus on the problem that in the process of using LLM for KGC reordering, problems such as mismatches, misordering, and omissions may be encountered. To this end, KC-GenRe, a knowledge constraint generative KGC reordering method based on LLM, is introduced. To overcome the mismatch problem, the KGC reordering task is formulated as a candidate identifier sorting generation problem implemented by generative LLM. To address the misordering problem, a knowledge-guided interactive training method is developed, which improves the identification and ranking of candidates. To address the omission problem, a knowledge-enhanced constraint inference method is designed to enable context prompting and control generation for effective ranking. KG-GenRe achieved gains of up to $6.7\%$ and $7.7\%$ on the MRR and Hits@1 indicators on the four datasets compared to the previous method, and up to $9.0\%$ and $11.1\%$ compared to the non-reordered method. 
Description-based KGC, which leverages pre-trained language models (PLMs) to learn entity and relation representations with their names or descriptions, is limited by the quality of text and the incomplete structure \cite{DBLP:conf/coling/XuZLWZ000C24}. To address this issue, \cite{DBLP:conf/coling/XuZLWZ000C24} propose MPIKGC, a general framework to compensate for the deficiency of contextualized knowledge and improve KGC by querying large language models (LLMs) from various perspectives, which involves leveraging the reasoning, explanation, and summarization capabilities of LLMs to expand entity descriptions, understand relations, and extract structures, respectively. 
To overcome the challenge that the static and noisy nature of existing corpora generally limits the potential of PLM-based KGC models, \cite{DBLP:conf/eacl/LiTCL24} introduces the Contextualization Distillation strategy, a versatile plug-and-play approach that is compatible with both discriminative and generative KGC frameworks. The approach first instructs LLMs to transform compact structural triples into context-rich fragments, and then introduces two customized auxiliary tasks - reconstruction and contextualization - that allow smaller KGC models to absorb insights from these rich triplets. 
To alleviate the low efficiency of text-based KGC and the long-tail entities problems of triple-based KGC, \cite{DBLP:conf/emnlp/WeiH0K23} proposes KICGPT, a framework that integrates a large language model (LLM) and a triple-based KGC retriever. KICGPT uses an in-context learning strategy called Knowledge Prompt, which encodes structural knowledge into demonstrations to guide the LLM. It alleviates the long-tail problem without incurring additional training overhead.
In addition, \cite{DBLP:journals/corr/abs-2310-08279} analyzed to verify the hypothesis that LLMs, without fine-tuning, can refine entity descriptions, serving as an auxiliary knowledge source. It found that without fine-tuning, LLMs can further improve the quality of entity text descriptions.  LLMs exhibit text-generation hallucination issues and selectively output words with multiple meanings, which can be mitigated by contextualizing prompts to constrain LLM outputs. Larger model sizes do not necessarily guarantee better performance, even the 7B model can achieve optimized results in this comparative task. These findings underscore the untapped potential of large models in text-based KGC, which is a promising direction for further research in KGC.


These works demonstrate that LLMs could be utilized to complete current knowledge graphs, either by extracting knowledge from parameters of the LLMs or enhancing the reasoning capabilities of predicting missing triples. 








==> tables/comparison.tex <==
\begin{table}[]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l l l }
    \toprule
         & LM-as-KB & Conventional Structured KB & LLMKG  \\
         \midrule 
         \textbf{Construction} & Self/Unsupervised \thumbsup & Manual or semi-automatic \thumbsdown & Automatic \thumbsup \\
         \textbf{Schema} & Open-ended \thumbsup & Typically fixed \thumbsdown & Open-ended \thumbsup \\
         \textbf{Maintenance} \\
         - adding facts & Difficult, upredictable side effects \thumbsdown & Easy \thumbsup & Easy \thumbsup \\
         - correcting/deleting & Difficult \thumbsdown & Easy \thumbsup  & Easy \thumbsup \\
         \textbf{Knows what it knows} & No, assigns probability to everything \thumbsdown & Yes, content enumerable \thumbsup & Yes, content enumerable \thumbsup \\
         % \textbf{Entity disambiguation} & No/limited \thumbsdown & Common \thumbsup \\
         \textbf{Provenance} & No \thumbsdown & Common \thumbsup & Common \thumbsup\\
         \bottomrule
    \end{tabular}
    }
    \caption{Difference of LM-as-KBs, structured KBs and LLMKG.}
    \label{tab:difference}
\end{table}
